Time-Travel Investigation: Towards Building A Scalable Attack Detection Framework on Ethereum

As one of the representative blockchain platforms, Ethereum has attracted lots of attacks. Due to the existed financial loss, there is a pressing need to perform timely investigation and detect more attack instances. Though multiple systems have been proposed, they suffer from the scalability issue due to the following reasons. First, the tight coupling between malicious contract detection and blockchain data importing makes them infeasible to repeatedly detect different attacks. Second, the coarse-grained archive data makes them inefficient to replay transactions. Third, the separation between malicious contract detection and runtime state recovery consumes lots of storage. In this paper, we present the design of a scalable attack detection framework on Ethereum. It overcomes the scalability issue by saving the Ethereum state into a database and providing an efficient way to locate suspicious transactions. The saved state is fine-grained to support the replay of arbitrary transactions. The state is well-designed to avoid saving unnecessary state to optimize the storage consumption. We implement a prototype named EthScope and solve three technical challenges, i.e., incomplete Ethereum state, scalability, and extensibility. The performance evaluation shows that our system can solve the scalability issue, i.e., efficiently performing a large-scale analysis on billions of transactions, and a speedup of around 2,300x when replaying transactions. It also has lower storage consumption compared with existing systems. The result with three different types of information as inputs shows that our system can help an analyst understand attack behaviors and further detect more attacks. To engage the community, we will release our system and the dataset of detected attacks.

==> figures/df_anomies.tex <==
\begin{figure}[t]
    \includegraphics[width=0.57\textwidth]{pdfs/defianomie.pdf}
    \caption{The distribution of internal transaction number and ERC20 token transfer times for each normal transaction.
    The x-axis represents the number of internal transactions for each normal transaction; the y-axis represents
the times of ERC20 token transfer for each normal transaction. Each box in the graph represent a two-dimensional interval ($x1 < x < x2$ and $y1 < y < y2$), and the number $n$ in the box indicate
there exist $n$ normal transactions with the $x$ and $y$ dropped in the interval. The color of the box becomes darker as $x$ and $y$
become larger. }
    \label{fig:df_anomies}
\end{figure}


==> figures/df_defi_attack_graph.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{pdfs/defi_attack.pdf}
    \caption{The attack flow. Square: EOA, Circle: smart contract; Grey box: attacker, Red Box: victim;}
    \label{fig:df_attackflow}
\end{figure}


==> figures/df_workflow.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\textwidth]{pdfs/detectionflow.pdf}
    \caption{Detection workflow.}
    \label{fig:df_workflow}
\end{figure}


==> tables/eva_multithreading.tex <==
\begin{table}
	\centering
	
	\footnotesize
	\caption{Performance gain of using multithreading.}
	\label{tab:eva_perfmultithread}
	\begin{tabular}{|l|l|l|}
		\hline
		& Group $1$ & Group $2$ \\
		\hline
		\textbf{Single thread} & $1 m 42 s 358 ms$ & $0 m 14 s 802 ms$ \\
		\hline
		\textbf{Multithreading} & $0 m 12 s 458 ms$ & $ 0 m 1 s 570 ms $ \\
		\hline
	\end{tabular}
	\begin{tablenotes}
		\item Group 1: $1000$ normal transactions that will trigger more than $20$ internal transactions;
		\item Group 2: $1000$ simple normal transactions that will trigger only one internal transaction.
	\end{tablenotes}
\end{table}

==> tables/eva_overall_result.tex <==
\begin{table}
    \centering
    \caption{The overall result of attacks' instances detected by our system. ({NOR: normal transaction. INT: internal transactions. EOA: externally owned account. CON:contract account.})}
    \label{tab:eva_overallresult}
    \resizebox{.45\textwidth}{!}{
    \begin{tabular}{|l|l|l|l|}
    \hline
    \textbf{\# of Blocks} & \textbf{\# of Transactions} & \multicolumn{2}{c|}{\textbf{\# of Accounts}} \\
    \hline
    $10.4M$ & NOR $754,614,255$ & \multicolumn{2}{c|}{EOA: $95,769,440$} \\
     & INT: $962,171,044$ & \multicolumn{2}{c|}{CON: $27,361,936$} \\
    \hline
    \hline
    \textbf{Attack Types} &
    \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{\# of Malicious}\\\textbf{Transactions}\end{tabular}} &
    \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{\# of }\\\textbf{Victims}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{\# of }\\\textbf{Attackers}\end{tabular}} \\
    
    \hline
    {\textit{Suicide Bomb}} & NOR: $38,840$ &\multirow{2}{*}{\diagbox[width=1.80cm, height=0.55cm]{}} & EOA: $43$\\
    {DoS Attack} & INT: $19,154,939$ &&CON: $104$\\
    \hline
    {AirDrop Hunting} & NOR: $103,901$ & EOA: $0$&$26,976$\\
    {Attack} & INT: $10,261,383$ & CON: $363$&$10,36$\\
    \hline
    {Re-entrancy} & NOR: $2,973$ &EOA: $0$&$91$\\
    {Attack} & INT: $436,291$ &CON: $51$&$92$\\
    \hline
    {Bad Randomness} & NOR: $40,449$ &EOA: $0$ &$272$\\
    {Attack} & INT: $808,308$ &CON: $102$ &$229$\\
    \hline
    {EXTCODESIZE} & NOR: $3,221$ &\multirow{2}{*}{\diagbox[width=1.80cm, height=0.55cm]{}}& EOA: $22$\\
    {DoS Attack} & INT: $125,952$ &&CON: $1$\\
    \hline
    {Integer Overflow} & NOR: $506$ &EOA: $0$&$115$\\
    {Attack} & INT: $492$ &CON: $38$&$0$\\
    \hline
    {Short Address} & NOR: $240$ &EOA: $35$ &$48$\\
    {Attack} & INT: $35$ & CON: $0$&$0$\\
    \hline
    \end{tabular}}
    \begin{tablenotes}
    \item The evaluation is performed on the first 10,400,000 blocks. The table shows the number of attacks' instances detected by \system{}. 
    We also show the number of victim accounts that have been exploited and attacker accounts.
    \end{tablenotes}
\end{table}

